A Reinforcement Learning Framework for Dynamic Mediation Analysis

Mediation analysis learns the causal effect transmitted via mediator variables between treatments and outcomes and receives increasing attention in various scientific domains to elucidate causal relations. Most existing works focus on point-exposure studies where each subject only receives one treatment at a single time point. However, there are a number of applications (e.g., mobile health) where the treatments are sequentially assigned over time and the dynamic mediation effects are of primary interest. Proposing a reinforcement learning (RL) framework, we are the first to evaluate dynamic mediation effects in settings with infinite horizons. We decompose the average treatment effect into an immediate direct effect, an immediate mediation effect, a delayed direct effect, and a delayed mediation effect. Upon the identification of each effect component, we further develop robust and semi-parametrically efficient estimators under the RL framework to infer these causal effects. The superior performance of the proposed method is demonstrated through extensive numerical studies, theoretical results, and an analysis of a mobile health dataset.

==> Original_Version/1._Introduction.tex <==
\section{Introduction}
\textbf{Motivation:} From the perspective of mental health

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figure/Standard MDP.jpg}}
\caption{Standard MDP.}
\label{fig:Standard MDP}
\end{center}
\vskip -0.2in
\end{figure}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figure/Proposed MDP.jpg}}
\caption{Mediated MDP.}
\label{fig:Proposed MDP}
\end{center}
\vskip -0.2in
\end{figure}

==> Original_Version/2._Data_and_Problem_Formulation.tex <==
\section{Data and problem formulation}
We start with a simple formulation where the data consist of the state-action-mediator-reward tuples $\{(S_t,A_t,M_t,R_t):t\ge 0\}$. We adopt a reinforcement learning framework to formulate the mediation effects evaluation problem. Suppose there exists an agent that tries to learn and interact with a given environment. At each time $t$, the environment arrives at a state $S_t$. The agent selects an action $A_t$ according to the behavior policy $\pi_b(\bullet|S_t)$.
%The data generating process can be described as follows. At each time, the agent selects an treatment $A_t$. 
The mediator $M_t$ is drawn according to $p_m(\bullet|S_t,A_t)$ and the next-state $S_{t+1}$ and outcome $R_t$ are generated according to $p_{s',r}(\bullet,\bullet|S_t,A_t,M_t)$. %Suppose the treatment is binary and is fixed to $0$ at the initial time point, i.e., $A_0=0$. Let $\nu$ denote the initial mediator distribution. We are interested in learning the dynamic mediation effect under this setup. 



\section{Effect Estimation}
We first define the dynamic mediation effect. Consider the causal effect
\begin{eqnarray*}
	\textrm{ATE}=\lim_{T\to \infty} \frac{1}{T}\sum_{t=0}^{T-1} (\Mean^{\pi_e} R_t - \Mean^{a_0} R_t),
\end{eqnarray*}
where $\Mean^{\pi}$ denotes the expectation by assuming that %the treatment $a$ is repeatedly assigned all the time. 
the system follows a given stationary policy $\pi$ and $a_0$ denotes a nondynamic policy that assigns a fixed treatment $a_0$ all the time. In practice, to meet the Markov assumption, we can set $S_t$ to be the past data observations. 
For instance, in the intern health study, suppose we primarily focus on interns' mental health conditions. The reward corresponds to the mood score, the mediator corresponds to the step counts and sleep hours, the action corresponds to the text message, and the state corresponds to the mediator-reward pair in the past. 


Using the importance sampling method, we can represent ATE by
\begin{eqnarray*}
	&&\textrm{ATE}=\Mean \omega^{\pi_e}(S_t) \frac{\pi_e(A_t|S_t)}{\pi_b(A_t|S_t)}R_t-\Mean \omega^{a_0}(S_t) \frac{\mathbb{I}(A_t=a_0)}{\pi_b(A_t|S_t)}R_t\\
	&=&\sum_m \Mean \left[ \omega^{\pi_e}(S_t) \frac{\pi_e(A_t|S_t)}{\pi_b(A_t|S_t)}-\omega^{a_0}(S_t) \frac{\mathbb{I}(A_t=a_0)}{\pi_b(A_t|S_t)} \right] r(S_t,A_t,m)p_m(m|S_t,A_t)\\
	&=&\sum_{a,m} \Mean[\pi_e(a|S_t)\omega^{\pi_e}(S_t) r(S_t,a,m)p_m(m|S_t,a) -\pi_0(a|S_t)\omega^{a_0}(S_t) r(S_t,a,m)p_m(m|S_t,a)]
\end{eqnarray*}
where $\omega^{\pi}$ denotes the probability ratio of the stationary distribution of $S_t$ under a given policy $\pi$ and that under the behavior policy, %the policy that repeatedly assigns $a$ and that under the behavior policy, 
and $r$ denotes the conditional expectation of $R_t$ given $(S_t,A_t,M_t)$. 

By definition, ATE can be decomposed into the following three terms
\begin{eqnarray*}
	&&\sum_{a,m} \Mean\omega^{\pi_e}(S_t) \pi_e(a|S_t) [r(S_t,a,m)-r(S_t,a_0,m)] p_m(m|S_t,a)\\
	&+&\sum_{a,m} \Mean\omega^{\pi_e}(S_t) \pi_e(a|S_t) r(S_t,a_0,m)  [ p_m(m|S_t,a)-p_m(m|S_t,a_0)]\\
	&+&\sum_{m} \Mean [\omega^{\pi_e}(S_t)-\omega^{a_0}(S_t)]r(S_t,a_0,m)p_m(m|S_t,a_0).
\end{eqnarray*}
\begin{eqnarray*}
	&&\sum_{a,m} \Mean\omega^{\pi_e}(S_t) \pi_e(a|S_t) [r(S_t,a,m)-\sum_{a'}r(S_t,a',m)\pi_0(a'|S_t)] p_m(m|S_t,a)\\
	&+&\sum_{a',m} \Mean\omega^{\pi_e}(S_t) \pi_0(a'|S_t) r(S_t,a',m)  [ \sum_{a}\pi_e(a|S_t)p_m(m|S_t,a)-p_m(m|S_t,a')]\\
	&+&\sum_{a'm} \Mean [\omega^{\pi_e}(S_t)-\omega^{a_0}(S_t)] \pi_0(a'|S_t) r(S_t,a',m) p_m(m|S_t,a').
\end{eqnarray*}
Here, the first term denotes the direct effect of the treatment (DE), the second term denotes the indirect effect of the mediator (ME) and the last term denotes the indirect effect of the state (SE). It also outlines three estimators for these three treatment effects. 

We next derive the most efficient estimator for each causal effect. 
Define the Q-function
\begin{eqnarray}\label{Q:pi_e}
	Q^{\pi_e}(s,a,m)=\sum_{t\ge 0} \Mean^{\pi_e} [R_t-\eta^{\pi_e}|M_0=m,A_0=a,S_0=s],
\end{eqnarray}
where $\eta^{\pi_e}$ denotes the average reward under $\pi_e$. Define another Q-function as follows,
\begin{eqnarray*}
	Q^{\pi_e,a_0}(s,a,m)=\sum_{t\ge 0}\Mean^{\pi_e}  [r(S_t,a_0,M_t)-\eta^{\pi_e,a_0}|M_0=m,A_0=a,S_0=s],
\end{eqnarray*}
where $\eta^{\pi_e,a_0}=\eta^{\pi_e}-$DE.
%It satisfies the following Bellman equation,
%\begin{eqnarray*}
%	C^{\pi_e,\pi_0}(S_t,A_t,M_t)+\textrm{DE}=\Mean \left[\left.\frac{\pi_e(A_t|S_t)-\mathbb{I}(A_t=a_0)}{\pi_b(A_t|S_t)} R_t + C^{\pi_e,\pi_0}(S_{t+1},A_{t+1},M_{t+1})\right|A_t,S_t,M_t\right].
%\end{eqnarray*}


Consider DE. For a given $(S,A,M,R,S')$ tuple, the estimating function equals DE $+I_1-I_2$ where both $I_1$ and $I_2$ are augmentation terms, given by
\begin{eqnarray*}
	I_1=\omega^{\pi_e}(S) \frac{\pi_e(A|S)}{\pi_b(A|S)}\left[R+ \Mean_{\substack{a\sim \pi_e(\bullet|S')\\ m\sim p(\bullet|a,S')}} Q^{\pi_e}(S',a,m)-\Mean_{m\sim p(\bullet|A,S)}Q^{\pi_e}(S,A,m)-\eta^{\pi_e}\right]\\
	I_2=\omega^{\pi_e}(S) \left[ \frac{\sum_a \pi_e(a|S) p(M|S,a)}{p(M|S,A)}\frac{\mathbb{I}(A=a_0)}{\pi_b(A|S) }\{R-r(S,A,M)\}+\frac{\pi_e(A|S)}{\pi_b(A|S)}\right.\\
	\times \left.\{r(S,a_0,M)+\Mean_{\substack{a\sim \pi_e(\bullet|S')\\m\sim p(\bullet|S',a)}} Q^{\pi_e,a_0}(S',a,m)-\Mean_{m\sim p(\bullet|S,A)}Q^{\pi_e,a_0}(S,A,m)-\eta^{\pi_e,a_0}\}
	\right].
%	\\+\omega^{\pi_e}(S)\frac{\pi_e(A|S)}{\pi_b(A|S)}[Q^{\pi_e,a_0}(S,A,M)-\Mean_{m\sim p(\bullet|S,A)}Q^{\pi_e,a_0}(S,A,m) ].
\end{eqnarray*}
The purpose of adding these two augmentation terms is to reduce the bias of the direct estimator for DE. Consistency of the resulting estimator requires %$p_m$ to be correctly specified. However, either 
$(\omega^{\pi_e},\pi_b,r)$ or $(\omega^{\pi_e},\pi_b,p_m)$, or $(Q^{\pi_e}, Q^{\pi_e,a_0},\eta^{\pi_e},\eta^{\pi_e,a_0},r,p_m)$ to be consistently estimated. %is allowed to be misspecified. 

Next, consider ME. Define
\begin{eqnarray*}
	Q^{\pi_e,a_0*}(s,a,m)=\sum_{t\ge 0}\Mean^{\pi_e}  [\sum_m r(S_t,a_0,m)p(m|S_t,a_0)-\eta^{\pi_e,a_0*}|M_0=m,A_0=a,S_0=s],
\end{eqnarray*}
where $\eta^{\pi_e,a_0*}=\eta^{\pi_e,a_0}-$ME. 
The estimating function equals ME $+I_2-I_3$ where $I_3$ is an augmentation term, given by
\begin{eqnarray*}
	\omega^{\pi_e}(S)\left[\frac{\mathbb{I}(A=a_0)}{\pi_b(A|S)} \{R-\Mean_{m\sim p(\bullet|S,A)}r(S,A,m)\}+\frac{\pi^e(A|S)}{\pi^b(A|S)}\{\Mean_{m\sim p(\bullet|S,a_0)}r(S,a_0,m)\right.\\+\Mean_{\substack{a\sim \pi_e(\bullet|S')\\m\sim p(\bullet|S',a)}} Q^{\pi_e,a^*_0}(S',a,m)
	-\left.\Mean_{m\sim p(\bullet|S,A)} Q^{\pi_e,a^*_0}(S,A,m)-\eta^{\pi_e,a_0*}\}\right].
\end{eqnarray*}
%!TODO Check the $\Mean_{m\sim p(\bullet|S,A)}r(S,A,m)$ via EIF derivation.

Consistency of this estimator requires $(\omega^{\pi_e},\pi_b,r)$ or $(\omega^{\pi_e},\pi_b,p_m)$, or $( Q^{\pi_e,a_0},Q^{\pi_e,a_0*},\eta^{\pi_e,a_0},\eta^{\pi_e,a_0*},r,p_m)$ to be consistently estimated.


 Finally, consider SE. Define
 \begin{eqnarray*}
	Q^{a_0}(s,a,m)=\sum_{t\ge 0} \Mean^{a_0} [R_t-\eta^{a_0}|M_0=m,A_0=a,S_0=s],
\end{eqnarray*}
 where $\eta^{a_0} = \eta^{\pi_e,a_0*}-SE$ is the the average reward under $a_0$. The estimating equation equals SE $+I_3-I_4$ where $I_4$ is an augmentation term, given by
 \begin{eqnarray*}
 	I_4=\omega^{a_0}(S) \frac{\mathbb{I}(A=a_0)}{\pi_b(A|S)}\left[R+ \Mean_{\substack{ m\sim p(\bullet|a_0,S')}} Q^{a_0}(S',a_0,m)-\Mean_{m\sim p(\bullet|A,S)}Q^{a_0}(S,A,m)-\eta^{a_0}\right]
 \end{eqnarray*}
Similarly, this estimator is consistent when either $(\omega^{\pi_e},\pi_b,r)$ or $(\omega^{\pi_e},\pi_b,p_m)$, or $( Q^{\pi_e,a_0*},Q^{a_0},\eta^{\pi_e,a_0*},\eta^{a_0},r,p_m)$ is consistently estimated. 

 %Consider DE first. 
%Consider the discounted reward setting first. Meanwhile, our proposal can be extended to the average reward setting as well. Define the value function as the expected cumulative discounted reward 
%\begin{eqnarray*}
%	V^a(m)=\Mean^0 (R_0|M_0=m)+\sum_{t\ge 1} \gamma^t \Mean^a (R_t|M_0=m),
%\end{eqnarray*}
%where the expectation $\Mean^a$ is taken by assuming that all the actions after the initial time point are set to $a$. 


==> Original_Version/3._Related_Work.tex <==
\section{Related work}
(TBC)

\textbf{Ivan: Efficient and flexible causal mediation focus on the longitudinal data with multiple stages (our: infinite horizon )}
\begin{enumerate}
    \item Handle only categorical mediators; 

 \item All nodes from left to right: the distribution of A/M/L/Z are conditioned on all the past observations 

 \item The outcome of interest is the final reward, while we are interested in all the "time-varying covariates" 

 \item Exists intermediated confounders Z such that mediated the effect of A to M 

 \item Divided in total effect into indirect effect and the direct effect 

 \item $A_t$ = (Action, censoring) 
\end{enumerate}

\textbf{Tyler: Mediation analysis with time varying exposure (multiple stages, doubly robust)}

\textbf{Shi: "Off-Policy"} focus on value estimation instead of the mediation effect and assumes that Mt intercepts every directed path from A to R and S, M mainly used to block the unmeasured confounder.

\textbf{Liao:}

\begin{enumerate}
    \item Single stage mediation analysis
    \item Longtitudinal mediation analysis
    \begin{enumerate}
        \item No intermidiate reward, focusing on optimizing the final outcome \item M is categorical in most cases 
        \item The mediator at time t will not be affected by the outcome at time t-1
    \end{enumerate}
\end{enumerate}


 

==> Original_Version/4._Toy_Example.tex <==
\section{Toy Example}
Here, we show the triply robustness property of the proposed estimators, considering a setting with all the spaces of state, action, mediator, and reward are discrete valued.
\subsection{Data Generating Process}
\begin{align}
    S_{0}&\sim Bernoulli(0.5)\\
    M_{t}&\sim Bernoulli(expit(1.0-.5S_{t}+2.5A_{t}))\\
    R_{t}&\sim Bernoulli(expit(1.0+3.5S_{t}-3.0A_{t}+.5M_{t}))*10\\
    S_{t+1}&\sim Bernoulli(expit(.5+3.0S_{t}-2.5A_{t}-.5M_{t}))\\
    \pi_{b}&\sim Bernoulli(expit(1.0-2.0S{t}))\\
    \pi_{e}&\sim Bernoulli(expit(1.5+1.0S{t}))\\
    a_0&=0
\end{align}
We fix time $T=200$, and $S_{0}$ for each trajectory is sampled from a Bernoulli distribution with probability of $0.5$ and support $\{0,1\}$. Following the behavior policy, the action $A_{t} \in \{0,1\}$ is sampled from the Bernoulli distribution, where $\prob(A_{t} = 1|S_{t}) = expit(1.0-2.0S{t})$. Conditioned on $S_t$ and $A_{t}$, the mediator $M_{t} \in \{0,1\}$ is then randomly sampled from Bernoulli distribution with $\prob(M_{t} = 1|S_{t}, A_{t}) = expit(1.0-.5S_{t}+2.5A_{t})$. The distribution of $R_{t}$ and $S_{t+1}$ are conditional on $S_{t}$, $A_{t}$, and $M_{t}$, and are Bernoulli. The distribution of reward $R_{t}$ satisfies that $\prob(R_{t} = 10|S_{t}, A_{t}, M_{t}) = expit(1.0+3.5S_{t}-3.0A_{t}+.5M_{t})$, while the distribution of next state $S_{t+1}$ satisfied that $\prob(S_{t+1} = 1|S_{t}, A_{t}, M_{t}) = expit(.5+3.0S_{t}-2.5A_{t}-.5M_{t})$. We are interested in estimating the treatment effect between a target policy $\pi_e$, which takes a treatment $1$ with $\prob(A_{t} = 1|S_{t}) = expit(1.5+1.0S{t})$, and a fixed policy $a_0$, which assigns treatment $0$ all the time. 

The oracle distributions $\omega^{\pi_e}$, $\omega^{a_0}$, and the oracle values of $\eta^{\pi}$, $\eta^{\pi,a_0}$, $\eta^{\pi,a_0*}$, $\eta^{a_0}$ are derived by Monte Carlo simulations. Considering the true distribution of $Q^{\pi_e}$,$Q^{\pi_e,a0}$,$Q^{\pi_e,a0*}$,$Q^{a_0}$, we estimated them via the fitted Q-evaluation method \citep{le2019batch} with a linear regression model, respectively. Specifically, the estimation procedure is motivated by the Bellman equation model, such that:
\begin{align*}
    \Mean^{\pi_e}[R_{t}+\Mean_{m'}Q^{\pi_e}(S_{t+1},\pi_e(S_{t+1}),m')-\eta^{\pi}|S_{t}=s, A_{t}=a, M_{t}=m] = Q^{\pi_e}(S_{t},A_{t}, M_{t}),\\
    \Mean^{\pi_e}[r(s,a_0,m)+\Mean_{m'}Q^{\pi_e,a_0}(S_{t+1},\pi_e(S_{t+1}),m')-\eta^{\pi,a_0}|S_{t}=s, A_{t}=a, M_{t}=m] \\
    \left.= Q^{\pi_e,a_0}(S_{t},A_{t}, M_{t})\right.,\\
    \Mean^{\pi_e}[\Mean_{m'}r(s,a_0,m')+\Mean_{m*}Q^{\pi_e,a_0*}(S_{t+1},\pi_e(S_{t+1}),m*)-\eta^{\pi,a_0*}|S_{t}=s, A_{t}=a, M_{t}=m]\\
    \left.= Q^{\pi_e,a_0*}(S_{t},A_{t}, M_{t})\right.,\\
    \Mean^{a_0}[R_{t}+\Mean_{m'}Q^{a_0}(S_{t+1},a_0,m')-\eta^{a_0}|S_{t}=s, A_{t}=a, M_{t}=m] = Q^{a_0}(S_{t},A_{t}, M_{t}).
\end{align*}

To investigate the robustness of the proposed estimator, we evaluate their performance under four scenarios: i) $\mathcal{M}_{1}$,$\mathcal{M}_{2}$, and $\mathcal{M}_{3}$ are all correctly specified; ii) only $\mathcal{M}_{1}$ is correctly specified; iii) only $\mathcal{M}_{2}$ is correctly specified; and iv) only $\mathcal{M}_{3}$ is correctly specified. To misspecify the $\omega^{\pi_e}$, we add .25 to the $\omega^{\pi_e}(S_{t}=1)$ and subtract .25 from the $\omega^{\pi_e}(S_{t}=0)$. Similarly, we subtract .3 from the $\omega^{a_0}(S_{t}=1)$ and add .3 from the $\omega^{a_0}(S_{t}=0)$.


\subsection{Results}

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{Figure/robustness.png}
    \includegraphics[width=\columnwidth]{Figure/MSE.png}
    \caption{Robustness}
    \label{fig:robust}
\end{figure}

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\textwidth]{Figure/robustness_1.png}
%    \includegraphics[width=\textwidth]{Figure/MSE_1.png}
%%    \caption{Robustness}
%    \label{fig:robust}
%\end{figure}

\begin{align}
    DE = -3.88580387\\
    ME = 0.12011923\\
    SE = -1.20948795
\end{align}


==> Original_Version/5._Method.tex <==
\subsection{Learning $Q$ functions \& $\omega$}

\textbf{Objective.} \begin{equation}
    argmin_{\eta^{\pi_e},Q^{\pi_e}}T^{-1}\sum_{t=1}^{T}\big[R+ \Mean_{\substack{a\sim \pi_e(\bullet|S')\\ m\sim p(\bullet|a,S')}} Q^{\pi_e}(S',a,m)-\Mean_{m\sim p(\bullet|A,S)}Q^{\pi_e}(S,A,m)\big]^{2}-\eta^{\pi_e}
\end{equation}

\textbf{Coupled Estimation.} 
\begin{equation}
    argmin_{\eta^{\pi_e},Q^{\pi_e}}T^{-1}\sum_{t=1}^{T}\hat{g}_{i}^{2}(A_t,S_t,M_t;\eta^{\pi_e},Q^{\pi_e})+\lambda\|Q^{\pi_e}\|^{2},
\end{equation}where
\begin{multline}
    \hat{g} = argmin_{g}T^{-1}\sum_{t=1}^{T}\big[R+ \Mean_{\substack{a\sim \pi_e(\bullet|S')\\ m\sim p(\bullet|a,S')}} Q^{\pi_e}(S',a,m)-\Mean_{m\sim p(\bullet|A,S)}Q^{\pi_e}(S,A,m)-\eta^{\pi_e}\\
    -g(A_{t},S_{t},M_{t})\big]^{2}+\mu\|g\|^{2},
\end{multline}
Considering the class of linear regression, let 
\begin{align}
    g(A_{t},S_{t},M_{t}) & = [1,S_t,A_t,M_t]\beta = \boldsymbol{z}_t\beta \\
    Q^{\pi_e}(S_t,A_t,M_t) & = [S_t, A_t, M_t]\theta =\tilde{\boldsymbol{z}_t}\theta.
\end{align}
Therefore, we can rewrite the $\hat{g}$ as
\begin{multline}
    argmin_{\beta}\frac{1}{NT}\sum_{i,t}\Big\{R_{i,t}+\Mean_{\substack{a\sim \pi_e(\bullet|S')\\ m\sim p(\bullet|a,S')}} Q^{\pi_e}(S',a,m)-\Mean_{m\sim p(\bullet|A,S)}Q^{\pi_e}(S,A,m)
    -\eta^{\pi_e}-\boldsymbol{z}_{i,t}\beta\Big\}^{2}+\mu\beta^{T}\beta.
\end{multline} The closed form expression of $\beta$ is 
\begin{align}
    \hat{\beta} = (\boldsymbol{Z}^{T}\boldsymbol{Z}+NT\mu\boldsymbol{I}_{p})^{-1}\boldsymbol{Z}^{T}(\boldsymbol{R}+\boldsymbol{Q}^{(2)}-\eta^{\pi_e}\boldsymbol{1}-\boldsymbol{Q}^{(1)}).
\end{align}
Then $\hat{g}(S_t,A_t,M_t) = \boldsymbol{z}_t\hat{\beta}$, and 
\begin{align}
    \frac{1}{NT}\sum_{i,t}\hat{g}^{2}(A_{i,t},S_{i,t},M_{i,t};\eta^{\pi_e},Q^{\pi_e}) = \frac{1}{NT} \beta^{T}\boldsymbol{Z}^{T}\boldsymbol{Z}\beta.
\end{align}
With $Q^{\pi_e}(S_t,A_t,M_t) = [S_t, A_t, M_t]\theta =\tilde{\boldsymbol{z}_t}\theta$, we have that
\begin{align*}
    \Mean_{m\sim p(\bullet|A,S)}Q^{\pi_e}(S,A,m) &= [S,A,\Mean(m|A,S)]\theta = \boldsymbol{\tilde{z}_{i,t}^{(1)}}\theta\\
    \Mean_{\substack{a\sim \pi_e(\bullet|S')\\ m\sim p(\bullet|a,S')}} Q^{\pi_e}(S',a,m) &= [S',\Mean^{\pi_{e}}(a|S'),\Mean^{\pi_e}(m|S')]\theta = \boldsymbol{\tilde{z}_{i,t}^{(2)}}\theta.
\end{align*} Therefore, 
\begin{align*}
    \Mean_{\substack{a\sim \pi_e(\bullet|S')\\ m\sim p(\bullet|a,S')}} Q^{\pi_e}(S',a,m)-\Mean_{m\sim p(\bullet|A,S)}Q^{\pi_e}(S,A,m) = (\boldsymbol{\tilde{z}_{i,t}^{(2)}}-\boldsymbol{\tilde{z}_{i,t}^{(1)}})\theta = \boldsymbol{\tilde{z}_{i,t}}\theta
\end{align*}
Let 
\begin{align*}
    \boldsymbol{G} = \boldsymbol{Z}(\boldsymbol{Z}^{T}\boldsymbol{Z}+NT\mu\boldsymbol{I}_{p})^{-1}\boldsymbol{Z}^{T}\boldsymbol{Z}(\boldsymbol{Z}^{T}\boldsymbol{Z}+NT\mu\boldsymbol{I}_{p})^{-1}\boldsymbol{Z}^{T},
\end{align*} and
\begin{align*}
    \alpha = [\theta^{T},\eta^{\pi_e}]^{T}.
\end{align*}
\begin{align}
    \hat{\alpha} = argmin_{\alpha} \frac{1}{NT}[\boldsymbol{R}+[\boldsymbol{\tilde{Z}}, -\boldsymbol{1}]\alpha]^{T}\boldsymbol{G}[\boldsymbol{R}+[\boldsymbol{\tilde{Z}}, -\boldsymbol{1}]\alpha]+\frac{1}{NT}\alpha^{T}\begin{bmatrix}
NT\lambda \boldsymbol{I}_p & \boldsymbol{0}\\
0 & 0
\end{bmatrix}\alpha.
\end{align}
The closed form expression of $\hat{\alpha}$ is then,
\begin{align}
    \hat{\alpha} = \Big\{[\boldsymbol{\tilde{Z}}, -\boldsymbol{1}]^{T}\boldsymbol{G}[\boldsymbol{\tilde{Z}}, -\boldsymbol{1}] + \begin{bmatrix}
NT\lambda \boldsymbol{I}_p & \boldsymbol{0}\\
0 & 0
\end{bmatrix}\Big\}^{-1}[\boldsymbol{\tilde{Z}}, -\boldsymbol{1}]^{T}\boldsymbol{G}\boldsymbol{R}
\end{align}

Binary A, the simplest linear regression. CV is required to decide the tuning parameter.






%fitted Q-evaluation Method \citep{le2019batch}, it can be showed that the Q-estimate is consistent \citep{fan2020theoretical}


%estimate the $\omega$ by solving the equation $L$

==> Original_Version/6._Theory_robust.tex <==
\begin{theorem}
\label{thm:robustDE}
\textbf{Robustness of DE.}
Suppose the process $\{S_{i,t}\}_{t\ge 0}$ is stationary, $\pi_{b}(A_{i,t}|S_{i,t})$, $\hat{\pi}_{b}(A_{i,t}|S_{it})$, $p_{m}(M_{i,t}|S_{i,t}, A_{i,t})$, and $\hat{p}_{m}(M_{i,t}|S_{i,t}, A_{i,t})$ are uniformly bounded away from $0$. The proposed estimators for DE is consistent and asymptotically normal if any one of the following conditions holds:
\begin{enumerate}
    \item $\mathcal{M}_{1} = (\omega^{\pi_e},\pi_b,r)$ is correctly specified,
    \item $\mathcal{M}_{2} = (\omega^{\pi_e},\pi_b,p_m)$ is correctly specified,
    \item $\mathcal{M}_{3} = ( Q^{\pi_e}, Q^{\pi_e,a_0}, \eta^{\pi_e}, \eta^{\pi_e,a_0}, r, p_m)$ is correctly specified.
\end{enumerate}
\end{theorem}

\begin{theorem}\label{thm:robustME}
\textbf{Robustness of ME.}
Suppose the process $\{S_{i,t}\}_{t\ge 0}$ is stationary, $\pi_{b}(A_{i,t}|S_{i,t})$, $\hat{\pi}_{b}(A_{i,t}|S_{it})$, $p_{m}(M_{i,t}|S_{i,t}, A_{i,t})$, and $\hat{p}_{m}(M_{i,t}|S_{i,t}, A_{i,t})$ are uniformly bounded away from $0$. The proposed estimators for ME is consistent and asymptotically normal if any one of the following conditions holds:
\begin{enumerate}
    \item $\mathcal{M}_{1} = (\omega^{\pi_e},\pi_b,r)$ is correctly specified,
    \item $\mathcal{M}_{2} = (\omega^{\pi_e},\pi_b,p_m)$ is correctly specified,
    \item $\mathcal{M}_{3} = ( Q^{\pi_e,a_0}, Q^{\pi_e,a_0*}, \eta^{\pi_e,a_0}, \eta^{\pi_e,a_0*}, r, p_m)$ is correctly specified.
\end{enumerate}
\end{theorem}

\begin{theorem}
\label{thm:robustSE}
\textbf{Robustness of SE.} Suppose the process $\{S_{i,t}\}_{t\ge 0}$ is stationary, $\pi_{b}(A_{i,t}|S_{i,t})$, $\hat{\pi}_{b}(A_{i,t}|S_{it})$, $p_{m}(M_{i,t}|S_{i,t}, A_{i,t})$, and $\hat{p}_{m}(M_{i,t}|S_{i,t}, A_{i,t})$ are uniformly bounded away from $0$. The proposed estimators for SE is consistent and asymptotically normal if any one of the following conditions holds:
\begin{enumerate}
    \item $\mathcal{M}_{1} = (\omega^{\pi_e},\pi_b,r)$ is correctly specified,
    \item $\mathcal{M}_{2} = (\omega^{\pi_e},\pi_b,p_m)$ is correctly specified,
    \item $\mathcal{M}_{3} = ( Q^{\pi_e,a_0*}, Q^{a_0}, \eta^{\pi_e,a_0*}, \eta^{a_0}, r, p_m)$ is correctly specified.
\end{enumerate}
\end{theorem}


Theorem \ref{thm:robustDE} Theorem \ref{thm:robustME} Theorem \ref{thm:robustSE} formally establish the triply robustness property of all the proposed estimators for DE, ME, and SE, respectively. To save the space, the proof of Theorems is deffered to the Appendix \ref{appendix:robust}.

==> Original_Version/OPE_estimators.tex <==
\section{Dynamic Treatment Effects Evaluation}
In this section, we first develop DM and IS estimators for each dynamic treatment effect, whose consistencies require %the correct  specification of certain 
a given set of nuisance functions to be correctly specified. %which is commonly unknown in practice. 
%Therefore, we further proposed a multiply-robust estimator via deriving the efficient influence function (EIF) in section \ref{TRE}. 
This motivates us to develop doubly or triply robust estimators in section \ref{TRE} whose consistencies only require either one of the two or three sets of nuisance functions to be correctly specified. 
To save space, the detailed estimation procedures for the nuisance functions are relegated to Appendix \ref{nuisance}.
%Finally, we discuss the estimating methods with more details.
\subsection{Direct Estimators}
The direct estimators are built upon the Q-functions. %Note that all the expectations in this subsection are conditional on the initial state-action-mediator tuple. 
We first start with some notations. Let $\Mean^{\pi}_{s,a,m}[\cdot]$ denotes the conditional expectation $\Mean^{\pi}[\cdot|S_0=s, A_0=a, M_0=m]$. For any function $f$, let $\Mean_{\pi,a}(f(S)) = \Mean_{a\sim \pi(\bullet|S)}(f(S))$, $\Mean_{\pi,a,m}(f(S)) = \Mean_{a\sim \pi(\bullet|S), m\sim p(\bullet|S,a)}(f(S))$, and $\Mean_{m}(f(S,A)) = \Mean_{m\sim p(\bullet|S,A)}(f(S,A))$. For convenience, let $\pi_{a_0}^{m_e}$ denote the process in which we intervene to set actions by following $\pi_0$ and set mediators by randomly drawing from conditional distributions induced by $\pi_e$.
%This notation only applies to this subsection.

\textbf{Direct Estimator for $\textrm{IDE}(\pi_e,\pi_0)$.}
Define the Q-function 
\begin{equation*}\label{Q:pi_e}
Q^{\pi_e}(s,a,m) = \sum_{t\ge 0} \Mean^{\pi_e} [R_{t}-\eta^{\pi_e}|S_0=s, A_0=a, M_0=m],
\end{equation*}where $\eta^{\pi_e}$ denotes the average reward under $\pi_e$. Then, we define another Q-function $Q^{\pi_e,\pi_0}(s,a,m)$,
\begin{equation*}
	\sum_{t\ge 0}\Mean^{\pi_e}  [\Mean_{\pi_0,a^*}r(S_{t},a^*,M_{t})-\eta^{\pi_e,\pi_0}|S_0=s, A_0=a, M_0=m],
\end{equation*}
where $\eta^{\pi_e,\pi_0}$ is the expected value of $\Mean_{\pi_0,a^*}r(S_{t},a^*,M_{t})$ under policy $\pi_e$. Therefore, $\textrm{IDE}(\pi_e,\pi_0)=\eta^{\pi_e}-\eta^{\pi_e,\pi_0}$.
%$\sum_{a'}r(S_t,a',M_t)\pi_0(a'|S_t)$

\textbf{Direct Estimator for $\textrm{IME}(\pi_e,\pi_0)$.}
Similarly, we define $Q^{\pi_e,\pi_0^*}(s,a,m)$ as
\begin{equation*}
	\sum_{t\ge 0}\Mean^{\pi_e} [\Mean_{\pi_0,a^*,m^*} r(S_t,a^*,m^*)-
	\eta^{\pi_e,\pi_0^*}|S_0=s, A_0=a, M_0=m],
\end{equation*}
where the $\eta^{\pi_e,\pi_0^*}$ is the expectation of $\Mean_{\pi_0,a^*,m^*} r(S_t,a^*,m^*)$ under $\pi_e$. By definition, we then have that $\textrm{IME}(\pi_e,\pi_0)=\eta^{\pi_e,\pi_0}-\eta^{\pi_e,\pi_0^*}$. 
%$\int_m\sum_{a} r(S_t,a,m)p(m|S_t,a)\pi_0(a|S_t)$

\textbf{Direct Estimator for $\textrm{DDE}(\pi_e,\pi_0)$.} Considering the process $\pi_{a_0}^{m_e}$, we define $Q^{\pi_{a_0}^{m_e}}(s,a,m)$ as
\begin{equation*}
    \sum_{t\geq 0} \Mean^{\pi_{a_0}^{m_e}}[\Mean_{\pi_0,a^*,m^*} r(S_t,a^*,m^*)-\eta^{\pi_{a_0}^{m_e},\pi_0^*}|S_0=s, A_0=a, M_0=m],
\end{equation*} where $\eta^{G}$ is the expectation of $\Mean_{\pi_0,a^*,m^*} r(S_t,a^*,m^*)$ under the treatment process and the intervened mediator process of $G$. By definition, $\textrm{DDE}(\pi_e,\pi_0)=\eta^{\pi_e,\pi_0^*}-\eta^{G,\pi_0^*}$.
%$\sum_{m,a}p_{\theta_0}(m|S_t,a)r_{\theta_0}(S_t,a,m)\pi_0(a|S_t)$

\textbf{Direct Estimator for $\textrm{DME}(\pi_e,\pi_0)$.}
Similar to $Q^{\pi_e}(s,a,m)$, we define
 \begin{equation*}
	Q^{\pi_0}(s,a,m)=\sum_{t\ge 0} \Mean^{\pi_0} [R_t-\eta^{\pi_0}|S_0=s, A_0=a, M_0=m],
\end{equation*}
 where $\eta^{\pi_0}$ is the average reward under $\pi_0$. By definition, $\textrm{DME}(\pi_e,\pi_0) = \eta^{G,\pi_0^*}-\eta^{\pi_0}$.
 
These representations motivate us to learn $r$ and $p_m$ using the observed data and then plug in the estimated reward and mediator functions in order to learn each of the $Q$ functions with estimated $\eta$s as byproducts. Then, by plugging in estimated $\eta$s, the direct estimate of each effect is constructed.

\subsection{Importance Sampling (IS) Estimators}As commented earlier, standard IS estimators suffer from the curse of horizon. In this section, we utilize the marginal importance sampling (MIS) method proposed in \citet{liu2018breaking} to break the curse of horizon. %construct unbiased estimators with marginal importance ratio. %Let $\Mean^{\pi}$ be the expectation taken over $S_t$, which is following the stationary state distribution under policy $\pi$ (i.e., $p^{\pi}(S_t)$).
%We can rewrite each potential reward involved in the decomposition by using the state distribution. Specifically, 
For a given policy $\pi$, we first introduce the MIS ratio, given by
$$\omega^{\pi}(s) = \frac{p^{\pi}(s)}{p^{\pi_b}(s)}.$$
%where $p^{\pi}$ and $p^{\pi_b}$ denote the stationary state distribution under $\pi$ and $\pi_b$, respectively. 
Using the change of measure theorem, it is immediate to see that
\begin{eqnarray*}
    \frac{1}{NT}\sum_{i,t} \omega^{\pi_e}(S_{i,t})\frac{\pi_e(A_{i,t}|S_{i,t})}{\pi_b(A_{i,t}|S_{i,t})}R_{i,t},\\
    \frac{1}{NT}\sum_{i,t} \omega^{\pi_0}(S_{i,t})\frac{\pi_0(A_{i,t}|S_{i,t})}{\pi_b(A_{i,t}|S_{i,t})}R_{i,t},
\end{eqnarray*}
are unbiased to $\eta^{\pi_e}$ and $\eta^{\pi_0}$, respectively. 

\begin{comment}
For any arbitrary policy $\pi$ that results in stationary process $\{S_t\}_{t>0}$, let $p^{\pi}(S_t)$ denote the probability of $S_t$ under $\pi$.
%$\Mean \left[R^{*}_t(\pi,\bar{M}^{*}_{t}(\pi))\right]$ can be represented as
%\begin{align}\label{eqn:expected_potential_0}
%     \sum_{a}\int_{m} \Mean^{\pi} \pi(a|S_t) p_m(m|S_t,a) r(S_t,a,m).
%\end{align}
Let $\omega^{\pi}(s) = \frac{p^{\pi}(s)}{p^{\pi_b}(s)}$ be the probability ratio of the distribution of $S_t$ under a stationary policy $\pi$ and that under the behavior policy $\pi_b$. Let $\rho(S,A,M) = \frac{\sum_a \pi_e(a|S) p(M|S,a)}{p(M|S,A)}$. An IS-based estimator for $\Mean \left[R^{*}_t(\pi,\bar{M}^{*}_{t}(\pi))\right]$ is 
\begin{align*}
     \frac{1}{NT}\sum_{i,t} \omega^{\pi}(S_{i,t})\frac{\pi(A_{i,t}|S_{i,t})}{\pi_b(A_{i,t}|S_{i,t})}R_{i,t}.
\end{align*} 
%\begin{align*}\label{eqn:expected_potential_0}
%     \sum_{a}\int_{m} \Mean^{\pi_b} \omega^{\pi_e}(S_t) \pi_e(a|S_t) p_m(m|S_t,a) r(S_t,a,m).
%\end{align*}
\end{comment}
Similarly, we can show that there are two different IS-based ways to estimate $\Mean\left[R^{*}_t\left(\pi_{e,0}^{t},\bar{M}^{*}_{t}(\pi_e)\right)\right]$:
\begin{align*}
(\textrm{IS}_1) &: \frac{1}{NT}\sum_{i,t} \omega^{\pi_e}(S_{i,t}) \frac{\pi_0(A_{i,t}|S_{i,t})}{\pi_b(A_{i,t}|S_{i,t})} \rho(S_{i,t},A_{i,t},M_{i,t})R_{i,t},\\
(\textrm{IS}_2) &: \frac{1}{NT}\sum_{i,t} \omega^{\pi_e}(S_{i,t}) \frac{\pi_e(A_{i,t}|S_{i,t})}{\pi_b(A_{i,t}|S_{i,t})} \sum_{a}\pi_0(a|S)r(S,a,M).
\end{align*}
%where the outer expectation is taken over the distribution of $S_t$, $A_t$, $M_t$, and $R_t$.
%\begin{align*}
%\sum_{a,a'}\int_{m} \Mean^{\pi_b} \omega^{\pi_e}(S_t) \pi_0(a|S_t) r(S_t,a,m)\pi_e(a'|S_t)p(m|S_t,a'),
%\end{align*} 
Furthremore, an IS estimator of $\Mean\left[R^{*}_t\left(\pi_{e,0}^{t},\bar{M}^{*}_{t}(\pi_{e,0}^{t})\right)\right]$ is 
\begin{align*}
    \frac{1}{NT}\sum_{i,t} \omega^{\pi_e}(S_{i,t})\frac{\pi_0(A_{i,t}|S_{i,t})}{\pi_b(A_{i,t}|S_{i,t})} R_{i,t},
\end{align*} 
%\begin{align*}
%    \sum_{a}\int_{m} \Mean^{\pi_b}\omega^{\pi_e}(S_t) \pi_0(a|S_t) r(S_t,a,m) p_m(m|S_t,a).
%\end{align*}
and an IS estimator of $\Mean[R^{*}_t(\pi_{0},\bar{G}_{t}^{\pi_{e,0}^{t}})]$ is 
\begin{align*}
    \frac{1}{NT}\sum_{i,t} \omega^{G}(S_{i,t})\frac{\pi_0(A_{i,t}|S_{i,t})}{\pi_b(A_{i,t}|S_{i,t})} R_{i,t}.
\end{align*} 
The IS estimators for $\textrm{IDE}(\pi_e,\pi_0)$, $\textrm{IME}(\pi_e,\pi_0)$, $\textrm{DDE}(\pi_e,\pi_0)$, and $\textrm{DME}(\pi_e,\pi_0)$ are then obtained by plugging in the above expressions accordingly. 

As has been widely discussed in the literature, both the direct and IS estimators have limitations \citep{shi2022off}. First, as suggested by the estimator constructions, the consistency of direct estimators requires correct model specification of $r$, $p_m$, and $Q$ functions, while the consistency of IS estimators requires correct model specification of $\pi_b$, $p_m$, $\omega^{\pi_e}$, $\omega^{\pi_0}$, and $\omega^{G}$. %Second, in real practice, it is easy for direct estimators to be highly biased due to incorrect model specifications, while IS estimators are typically inefficient, with a variance strictly greater than the semi-parametric efficiency bound.
%direct estimators suffer from the bias introduced by model misspecification of $Q$, whereas IS estimators suffer from the large variance introduced by the estimation of importance weight \citep{liu2018breaking}. 
Therefore, in the next section, we further propose multiply-robust estimators with low bias and low variance to mitigate the limitations.




%\begin{equation}\label{eqn:expected_potential_0}
%\int_{m}\sum_{a,a'}\Mean^{\pi_1} r(S_t,a,m)p(m|S_t, a')\pi_2(a| S_t)\pi_3(a'|S_t)d_{m},
%\end{equation}

%\begin{equation*}
%\label{eqn:expected_potential_1}
%    \int_m\sum_{a,a'}\Mean^{\pi_b}\omega^{\pi_1}(S_t) r(S_t,a,m)\pi_2(a|S_t)p(m|S_t,a')\pi_3(a'|S_t)d_m,
%\end{equation*}
%where the outer expectation is taken over $S_t$ under $\pi_b$. 

%\begin{eqnarray*}
%	&&\sum_{a,m} \Mean\omega^{\pi_e}(S_t) \pi_e(a|S_t) [r(S_t,a,m)-\sum_{a'}r(S_t,a',m)\pi_0(a'|S_t)] p_m(m|S_t,a)\\
%	&+&\sum_{a',m} \Mean\omega^{\pi_e}(S_t) \pi_0(a'|S_t) r(S_t,a',m)  [ \sum_{a}\pi_e(a|S_t)p_m(m|S_t,a)-p_m(m|S_t,a')]\\
%	&+&\sum_{a'm} \Mean [\omega^{\pi_e}(S_t)-\omega^{a_0}(S_t)] \pi_0(a'|S_t) r(S_t,a',m) p_m(m|S_t,a').
%\end{eqnarray*}
%Here, the first term denotes the direct effect of the treatment (DE), the second term denotes the indirect effect of the mediator (ME) and the last term denotes the indirect effect of the state (SE). It also outlines three estimators for these three treatment effects. 


\subsection{Multiply Robust (MR) Estimators}\label{TRE}
%It satisfies the following Bellman equation,
%\begin{eqnarray*}
%	C^{\pi_e,\pi_0}(S_t,A_t,M_t)+\textrm{DE}=\Mean \left[\left.\frac{\pi_e(A_t|S_t)-\mathbb{I}(A_t=a_0)}{\pi_b(A_t|S_t)} R_t + C^{\pi_e,\pi_0}(S_{t+1},A_{t+1},M_{t+1})\right|A_t,S_t,M_t\right].
%\end{eqnarray*}
%We first start with some notations. 
Let $O$ denote a tuple $(S,A,M,R,S')$. This section presents the MR estimators %by introducing augmentation terms, which are combinations of 
that combine the DM and IS estimators. The process of derivation is based on EIF and is detailed in Appendix \ref{appendix:EIF}. 
% by introducing augmentation terms,

\textbf{MR-IDE.} To weaken the dependence on the correct model specification, we propose adding two augmentation terms, $I_1(O)$ and $I_2(O)$ to the direct estimator, which are appropriately constructed by combining the direct estimator and IS estimator. Specifically, $I_1(O)$ equals
\begin{multline*}
    \omega^{\pi_e}(S)\frac{\pi_e(A|S)}{\pi_b(A|S)}\Big[R+ \Mean_{\pi_e,a,m} Q^{\pi_e}(S',a,m)-\\
    \Mean_{m}Q^{\pi_e}(S,A,m)-\eta^{\pi_e}\Big],
\end{multline*} where the term in the bracket is a temporal difference error under the MMDP model and policy $\pi_e$, which has a mean zero conditional on $(S,A,M)$. Therefore, the expectation of $I_1(O)$ equals $0$ when $Q^{\pi_e}$, $\eta^{\pi_e}$, and $p_m$ are correctly specified. 
$I_2(O)$ equals
\begin{multline*}
    \omega^{\pi_e}(S)\Big[\frac{\pi_0(A|S)}{\pi_b(A|S)} \rho(S,A,M)\{R-r(S,A,M)\}\\+
   \frac{\pi_e(A|S)}{\pi_b(A|S)}\Big\{\Mean_{\pi_0,a'} r(S,a',M)+\Mean_{\pi_e,a,m} Q^{\pi_e,\pi_0}(S',a,m)\\-
	\Mean_{m}Q^{\pi_e,\pi_0}(S,A,m)-\eta^{\pi_e,\pi_0}\Big\}\Big],
\end{multline*} where the terms in both curly brackets have conditional mean equal to zero given $(S,A,M)$. Thus, $I_2(O)$ has zero mean when $r$, $p_m$, $Q^{\pi_e,\pi_0}$, and $\eta^{\pi_e,\pi_0}$ are correctly specified. Then the MR estimator of $\textrm{IDE}(\pi_e,\pi_0)$ is 
\begin{align}\label{eqn:IDE}
    \frac{1}{NT}\sum_{i,t}\eta^{\pi_e}-\eta^{\pi_e,\pi_0}+I_1(O_{i,t})-I_2(O_{i,t}).
\end{align} 
As discussed, when $(Q^{\pi_e}, Q^{\pi_e,\pi_0},\eta^{\pi_e},\eta^{\pi_e,\pi_0},r,p_m)$ are correctly specified, all the augmentation terms have mean zero, resulting in (\ref{eqn:IDE}) being identical to the direct estimator and therefore consistent. When $(\omega^{\pi_e},\pi_b,r)$ are correctly specified, the expectation of the sum of components involving $Q^{\pi_{e}}$, $Q^{\pi_{e},\pi_0}$, $\eta^{\pi_e}$, and $\eta^{\pi_e,\pi_0}$ equals zero, and the expectation of the first line of $I_2(O)$ is also zero. Then (\ref{eqn:IDE}) equals the IS estimator with $\textrm{IS}_2$ and is thus consistent. Similarly, when $(\omega^{\pi_e},\pi_b,p_m)$ are correctly specified, (\ref{eqn:IDE}) equals to the IS estimator with $\textrm{IS}_1$ and is hence consistent.

%The purpose of adding these two augmentation terms is to reduce the bias of the direct estimator for DE. 
%Consistency of the resulting estimator requires %$p_m$ to be correctly specified. However, either 
 %is allowed to be misspecified. 

\textbf{MR-IME.} Similarly, a MR estimator of $\textrm{IME}(\pi_e,\pi_0)$ is constructed by further introducing $I_3(O)$, which equals to
\begin{multline*}
	\omega^{\pi_e}(S)\Big[\frac{\pi_0(A|S)}{\pi_b(A|S)} \{R-\Mean_{m}r(S,A,m)\}+\\
	\frac{\pi_e(A|S)}{\pi_b(A|S)}\Big\{\Mean_{\pi_0, a',m}r(S,a',m)+\Mean_{\pi_e,a,m} Q^{\pi_e,\pi^*_0}(S',a,m)\\
	-
	\Mean_{m} Q^{\pi_e,\pi^*_0}(S,A,m)-\eta^{\pi_e,\pi_0^*}\Big\}\Big].
\end{multline*} The expectation of $I_3(O)$ is zero when $p_m$, $r$, $Q^{\pi_e,\pi_0^*}$, and $\eta^{\pi_e,\pi_0^*}$ are correctly specified. Then, the MR estimator of $\textrm{IME}(\pi_e,\pi_0)$ is specified as
\begin{align*}
    \frac{1}{NT}\sum_{i,t}\eta^{\pi_e,\pi_0}-\eta^{\pi_e,\pi_0^*}+I_2(O_{i,t})-I_3(O_{i,t}).
\end{align*} Following the same logic used for $I_2(O)$, consistency of this estimator is achieved when either $(\omega^{\pi_e},\pi_b,r)$ or $(\omega^{\pi_e},\pi_b,p_m)$, or $( Q^{\pi_e,\pi_0},Q^{\pi_e,\pi_0^*},\eta^{\pi_e,\pi_0},\eta^{\pi_e,\pi_0^*},r,p_m)$ is correctly specified.
%The estimating function equals  $\eta^{\pi_e,\pi_0}-\eta^{\pi_e,\pi_0^*}+I_2-I_3$ where $I_3$ is an augmentation term, given by
%!TODO Check the $\Mean_{m\sim p(\bullet|S,A)}r(S,A,m)$ via EIF derivation.

\textbf{MR-DDE.} Likewise, to construct the MR estimator of $\textrm{DDE}(\pi_e,\pi_0)$, we introduce $I_4(O)$ that equals
%and $\tilde{Q}^{G}(S,A,M)$ be 
%\begin{align*}
%    \int_{s',r'}\Big(\Mean^{G}_{a,m}Q^{G}(s',a,m)-\Mean^{G}_{m}Q^{G}(S,A,m)\Big)p(s',r'|S,A,M).
%\end{align*}
%$I_4(O)$ equals
\begin{multline*}
    \omega^{G}(S)\frac{\pi_0(A|S)}{\pi_{b}(A|S)}\Big[\Big\{R-\Mean_{m}r(S,A,m)\Big\}+\rho(S,A,M)\\
    \times
    \Big\{\Mean_{\pi_0, a',m}r(S,a',m)+ \Mean_{G,a,m}Q^{G}(S',a,m)\\-Q^{G}(S,A,M)-\eta^{G}\Big\}\Big]
    + \omega^{G}(S)\frac{\pi_e(A|S)}{\pi_{b}(A|S)}\\\times \sum_a \pi_0(a|S)\Big[Q^{G}(S,a,M)-\sum_m p(m|A,S)Q^{G}(S,a,m)\Big].
\end{multline*}
The MR estimator is then constructed as
 \begin{align*}
    \frac{1}{NT}\sum_{i,t}\eta^{\pi_e,\pi_0^*}-\eta^{G}+I_3(O_{i,t})-I_4(O_{i,t}),
\end{align*}
consistency of which requires either $(\omega^{\pi_e},\omega^{G},\pi_b,p_m)$, or $( Q^{G},Q^{\pi_e,\pi_0^*},\eta^{G},\eta^{\pi_e,\pi_0^*},r,p_m)$ to be consistently estimated.

\textbf{MR-DME.} Finally, we construct $I_5(O)$ to construct the MR estimator of $\textrm{DME}(\pi_e,\pi_0)$. $I_5(O)$ equals
\begin{multline*}
 	\omega^{\pi_0}\frac{\pi_0(A|S)}{\pi_b(A|S)}\Big[R+ \Mean_{\pi_0, a',m} Q^{\pi_0}(S',a',m)\\
 	-\Mean_{m}Q^{\pi_0}(S,A,m)-\eta^{\pi_0}\Big].
 \end{multline*} %which has a mean of zero when $\pi_b$, $p_m$, $Q^{\pi_0}$, and $\eta^{\pi_0}$ are correctly specified. 
 The MR estimator is then constructed as
 \begin{align*}
    \frac{1}{NT}\sum_{i,t}\eta^{G}-\eta^{\pi_0}+I_4(O_{i,t})-I_5(O_{i,t}).
\end{align*} Similarly, this estimator is consistent when either $(\omega^{\pi_0},\omega^{G},\pi_b,p_m)$, or $( Q^{G},Q^{\pi_0},\eta^{G},\eta^{\pi_0},r,p_m)$ are consistently estimated. 


%We would briefly state the triply robustness property in this section, and leave only the efficiency property to the Section 5.

 %Consider DE first. 
%Consider the discounted reward setting first. Meanwhile, our proposal can be extended to the average reward setting as well. Define the value function as the expected cumulative discounted reward 
%\begin{eqnarray*}
%	V^a(m)=\Mean^0 (R_0|M_0=m)+\sum_{t\ge 1} \gamma^t \Mean^a (R_t|M_0=m),
%\end{eqnarray*}
%where the expectation $\Mean^a$ is taken by assuming that all the actions after the initial time point are set to $a$. 





%\begin{multline*}
%    Q^{\pi_e,a_0}(S_{t},A_{t}, M_{t}) = \Mean^{\pi_e}[r(s,a_0,m)+\\
%    \Mean_{m'}Q^{\pi_e,a_0}(S_{t+1},\pi_e(S_{t+1}),m')
%    -\eta^{\pi,a_0}],
%\end{multline*}
%\begin{multline*}
%    Q^{\pi_e,a_0*}(S_{t},A_{t}, M_{t}) = \Mean^{\pi_e}[\Mean_{m'}r(s,a_0,m')+\\
%    \Mean_{m*}Q^{\pi_e,a_0*}(S_{t+1},\pi_e(S_{t+1}),m*)-\eta^{\pi,a_0*}],
%\end{multline*}
%\begin{multline*}
%    Q^{a_0}(S_{t},A_{t}, M_{t}) = \Mean^{a_0}[R_{t}+\Mean_{m'}Q^{a_0}(S_{t+1},a_0,m')\\
%    -\eta^{a_0}].
%\end{multline*}


==> name.tex <==
Mediation analysis learns the causal effect transmitted via mediator variables between treatments and outcomes, and receives increasing attention in various scientific domains to elucidate causal relations. Most existing works focus on point-exposure studies where each subject only receives one treatment at a single time point. However, there are a number of applications (e.g., mobile health) where the treatments are sequentially assigned over time and the dynamic mediation effects are of primary interest. Proposing a reinforcement learning (RL) framework, we are the first to evaluate dynamic mediation effects in settings with infinite horizons. We decompose the average treatment effect into an immediate direct effect, an immediate mediation effect, a delayed direct effect, and a delayed mediation effect. Upon the identification of each effect component, we further develop robust and semi-parametrically efficient estimators under the RL framework to infer these causal effects. The superior performance of the proposed method is demonstrated through extensive numerical studies, theoretical results, and an analysis of a mobile health dataset. A Python implementation of the proposed procedure is available at https://github.com/linlinlin97/MediationRL.

==> setup_summary.tex <==
\begin{itemize}
    \item $\pi_b(\bullet|S_t)$
    \item $p_m(\bullet|S_t,A_t)$
    \item $p_{s',r}(\bullet,\bullet|S_t,A_t,M_t)$
    \item Target: 
        \begin{eqnarray*}
    	&&\textrm{ATE}=\Mean \omega^{\pi_e}(S_t) \frac{\pi_e(A_t|S_t)}{\pi_b(A_t|S_t)}R_t-\Mean \omega^{a_0}(S_t) \frac{\mathbb{I}(A_t=a_0)}{\pi_b(A_t|S_t)}R_t\\
    	&=&\sum_m \Mean \left[ \omega^{\pi_e}(S_t) \frac{\pi_e(A_t|S_t)}{\pi_b(A_t|S_t)}-\omega^{a_0}(S_t) \frac{\mathbb{I}(A_t=a_0)}{\pi_b(A_t|S_t)} \right] r(S_t,A_t,m)p_m(m|S_t,A_t)\\
    	&=&\sum_{a,m} \Mean[\pi_e(a|S_t)\omega^{\pi_e}(S_t) r(S_t,a,m)p_m(m|S_t,a) -\pi_0(a|S_t)\omega^{a_0}(S_t) r(S_t,a,m)p_m(m|S_t,a)]
    	\end{eqnarray*}
    \item true Q, true w be solved by MC?
    \item $\eta^{\pi_{e}}$ by MC?
    把true model 放进去！for toy example 先不考虑Q estimation和别的estimation
\end{itemize}
